Beyond Gaze Points: Augmenting Eye Movement with Brainwave Data for Multimodal User Authentication in Extended Reality

Extended Reality (XR) technologies are becoming integral to daily life. However, password-based authentication in XR disrupts immersion due to poor usability, as entering credentials with XR controllers is cumbersome and error-prone. This leads users to choose weaker passwords, compromising security. To improve both usability and security, we introduce a multimodal biometric authentication system that combines eye movements and brainwave patterns using consumer-grade sensors that can be integrated into XR devices. Our prototype, developed and evaluated with 30 participants, achieves an Equal Error Rate (EER) of 0.29%, outperforming eye movement (1.82%) and brainwave (4.92%) modalities alone, as well as state-of-the-art biometric alternatives (EERs between 2.5% and 7%). Furthermore, this system enables seamless authentication through visual stimuli without complex interaction.

==> Section/05_Testbed.tex <==
%\section{Evaluation Setup}




==> Table/Tabel_FRM.tex <==

\begin{table*}
    \centering
    %\begin{tabular}{@{\extracolsep{1pt}}llllllll@{}}
    \begin{tabular}{clcccccc}
    %\begin{tabular}{>{\centering\arraybackslash\extracolsep{4pt}}m{3cm}*{6}{>{\centering\arraybackslash}m{2cm}}}
        \toprule
        \rowcolor[gray]{0.8}
        \multicolumn{2}{c}{\textbf{}} & 
        \multicolumn{2}{c}{\textbf{FRR at FAR = 1\%}} &
        \multicolumn{2}{c}{\textbf{FRR at FAR = 0.1\%}} & \multicolumn{2}{c}{\textbf{FRR at FAR = 0.0\%}} \\
        \cmidrule(r){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8}


        
        \textbf{Approach} & \textbf{Biometric}& \textbf{G 3} & \textbf{U 3} & \textbf{G 3} & \textbf{U 3} & \textbf{G 3} & \textbf{U 3} \\
        \midrule
        \multirow{3}{*}{\textbf{Single Biometric}} 
        & Brainwaves                 & 19.84 & 13.96 & 47.28 & 23.51  & 59.87 & 23.51\\ 
        & Eye-tracking with pupil    & 2.790 & 1.879 & 5.652 & 2.975 & 8.312  & 2.975\\
        & Eye-tracking without pupil & 7.466 & 9.192 & 27.71 & 18.03 & 34.47 & 18.03\\
        \midrule[1pt]
        \multirow{5}{*}{\textbf{Score Fusion}} 
       
        & Mean with pupil    & 0.000  & 0.180 & 0.360 & 0.270 & 0.811& 0.270 \\
        
        & Product with pupil & 0.000  & 0.000 & 0.178 & 0.000 & 0.448& 0.000 \\
        
        
        \cmidrule(l){2-8}

       
        & Mean without pupil    & 0.000 & 0.000 & 0.000 & 0.090 & 0.358 & 0.090\\
        
        & Product without pupil &0.000  & 0.090 & 0.360 & 0.180 & 0.718 & 0.180\\
        
        
        \midrule[1pt]
        \multirow{2}{*}{\textbf{Feature Fusion}} 

        & Architecture A with pupil & 0.087 & 0.360   &  1.880& 1.894 & 6.818 &1.894\\

        \cmidrule(l){2-8}
        
        & Architecture A without pupil & 0.541& 1.261 & 8.196 & 3.861 & 8.725 & 3.861\\

        \bottomrule
    \end{tabular}
    \caption{False Rejection Rate (FRR \%) at different False Rejection Rate FAR for Separated Biometrics, Score Fusion, and Feature Fusion Approaches under Different Comparison Scenarios.
    \matin{Not ready yet } 
    } 
    \label{T:EER}
    

\end{table*}

==> Table/Table_EER.tex <==
tr
\begin{table*}
    \centering
    %\begin{tabular}{@{\extracolsep{1pt}}llllllll@{}}
    \begin{tabular}{clcccccc}
    %\begin{tabular}{>{\centering\arraybackslash\extracolsep{4pt}}m{3cm}*{6}{>{\centering\arraybackslash}m{2cm}}}
        \toprule
        \rowcolor[gray]{0.8}
        \multicolumn{2}{c}{\textbf{}} & \multicolumn{3}{c}{\textbf{Global Fixed Threshold}} & \multicolumn{3}{c}{\textbf{User-Specific Threshold}} \\
        \cmidrule(r){3-5} \cmidrule(l){6-8}
        \textbf{Approach} & \textbf{Biometric}& \textbf{G 1} & \textbf{G 2} & \cellcolor{6} \textbf{G 3} & \textbf{U 1} & \textbf{U 2} & \cellcolor{6}\textbf{U 3} \\
        \midrule
        \multirow{3}{*}{\textbf{Single Biometric}} 
        & Brainwaves                 & 14.55 & 5.560 & 4.144 & 13.82  & 4.29 & 2.977\\ 
        & Eye-tracking with pupil    & \cellcolor{3} 13.42 &\cellcolor{3} 2.160&\cellcolor{3}1.180  &\cellcolor{3} 13.08 & \cellcolor{3}1.820 &\cellcolor{3} 0.798\\
        & Eye-tracking without pupil & 19.07 & 3.731 & 2.056 & 19.13 & 3.639 & 1.698\\
        \midrule[1pt]
        \multirow{5}{*}{\textbf{Score Fusion}} 
        
        & Max. with pupil    & 13.00 & 4.355 & 3.175 & 12.35 &3.762& 2.416\\
        
        & Min. with pupil    & 13.35 & 1.481 & 0.572 & 12.74 & 1.231& 0.383 \\
       
        & Mean with pupil    & 8.574 & 0.507 & 0.180 & 7.917 & 0.385& 0.034 \\
        
        & Product with pupil &\cellcolor{1} 7.098 & \cellcolor{1} 0.429 &\cellcolor{1} 0.123 & \cellcolor{1}6.683 &\cellcolor{1} 0.298&\cellcolor{1} 0.000 \\
        
        
        \cmidrule(l){2-8}
        
        & Max. without pupil    & 13.75 & 3.445 & 2.614 & 12.71 &2.990 & 1.382\\
        
        & Min. without pupil    & 13.85 & 1.510 & 0.472 & 13.87 & 1.350& 0.180\\
       
        & Mean without pupil    & 9.601 &\cellcolor{2} 0.850 & \cellcolor{2} 0.045 & 9.251 & \cellcolor{2} 0.686& \cellcolor{2} 0.011\\
        
        & Product without pupil & \cellcolor{2}9.281 & 0.906 & 0.079 & \cellcolor{2} 8.918 & 0.700 & 0.034 \\
        
        
        \midrule[1pt]
        \multirow{2}{*}{\textbf{Feature Fusion}} 

        & Architecture A with pupil & \cellcolor{4} 8.810 & \cellcolor{4} 0.917  & \cellcolor{4} 0.222 & \cellcolor{4} 7.817 & \cellcolor{4} 0.800 & \cellcolor{4} 0.055\\
        
        & Architecture B with pupil & 13.36 & 1.831 & 0.915 & 12.26 &  1.670 & 0.539\\ 

        \cmidrule(l){2-8}
        
        & Architecture A without pupil & \cellcolor{7} 10.47 &\cellcolor{7}  1.550 &\cellcolor{7} 0.619 &\cellcolor{7} 10.11 &\cellcolor{7} 1.230 &\cellcolor{7} 0.203\\
        
        & Architecture B without pupil & 16.28 & 4.373 & 2.189 & 15.82 & 4.080 & 1.434 \\

        \bottomrule
    \end{tabular}
    \caption{Equal Error Rates (EER \%) for Separated Biometrics, Score Fusion, and Feature Fusion Approaches under Different Comparison Scenarios.
    \matin{results need to be updated? U2 and G2, yes, but it will not be significant (expect to increase slightly} } 
    \label{T:EER}
    

\end{table*}
